pystacked: Stacking generalization and machine learning in Stata

pystacked implements stacked generalization (Wolpert, 1992) for regression and binary classification via Python's scikit-learn. Stacking combines multiple supervised machine learners -- the "base" or "level-0" learners -- into a single learner. The currently supported base learners include regularized regression, random forest, gradient boosted trees, support vector machines, and feed-forward neural nets (multi-layer perceptron). pystacked can also be used with as a `regular' machine learning program to fit a single base learner and, thus, provides an easy-to-use API for scikit-learn's machine learning algorithms.

==> Code/single_learner_2b.log.tex <==
. pystacked, type(reg) methods(gradboost) print
Default options: 
loss(squared_error) learning_rate(.1) n_estimators(100) subsample(1) criterion(friedman_mse) min_samples_split(2) min_samples_leaf(1) 
min_weight_fraction_leaf(0) max_depth(3) min_impurity_decrease(0) init(None) random_state(rng) max_features(None) alpha(.9) 
max_leaf_nodes(None) warm_start(False) validation_fraction(.1) n_iter_no_change(None) tol(.0001) ccp_alpha(0) 


==> Code/single_learner_2c.log.tex <==
. pystacked, type(reg) methods(lassocv) printopt
Default options: 
alphas(None) l1_ratio(1) eps(.001) n_alphas(100) fit_intercept(True) max_iter(1000) tol(.0001) 
n_jobs(None) positive(False) selection(cyclic) random_state(rng) 


==> Code/stack_reg_6.log.tex <==
. pystacked medh longi-medi                                   || ///
>     m(ols)                                                  || ///
>     m(ridgecv) xvars(c.(longi-medi)\#\#c.(longi-medi))        || ///
>     m(lassocv) xvars(c.(longi-medi)\#\#c.(longi-medi))        || ///
>     m(rf) opt(n_estimators(200))                            || ///
>     m(rf) opt(n_estimators(600))                            || ///
>     m(rf) opt(n_estimators(1000))                           || ///
>     m(gradboost) opt(n_estimators(200))                     || ///
>     m(gradboost) opt(n_estimators(600))                     || ///
>     m(gradboost) opt(n_estimators(1000))                    || ///
>     if train, type(regress) njobs(8)
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  ols            {\VBAR}      0.0000000
  ridgecv        {\VBAR}      0.0000000
  lassocv        {\VBAR}      0.0000000
  rf             {\VBAR}      0.1343528
  rf             {\VBAR}      0.1923578
  rf             {\VBAR}      0.1299185
  gradboost      {\VBAR}      0.0000000
  gradboost      {\VBAR}      0.0000000
  gradboost      {\VBAR}      0.5433710
{\smallskip}


==> pystacked for Stata/Code/single_learner_1.log.tex <==
. clear all
{\smallskip}
. use https://statalasso.github.io/dta/cal_housing.dta, clear
{\smallskip}
. set seed 42
{\smallskip}
. gen train=runiform()
{\smallskip}
. replace train=train<.75
(20,640 real changes made)
{\smallskip}
. replace medh = medh/10e3 
variable {\bftt{medhousevalue}} was {\bftt{long}} now {\bftt{double}}
(20,640 real changes made)


==> pystacked for Stata/Code/single_learner_2.log.tex <==
. pystacked medh longi-medi if train, type(reg) methods(gradboost)
Single base learner: no stacking done.
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  gradboost      {\VBAR}      1.0000000
{\smallskip}
. predict double yhat_gb1 if !train
{\smallskip}


==> pystacked for Stata/Code/single_learner_2b.log.tex <==
. pystacked, type(reg) methods(gradboost) print
Default options: 
loss(squared_error) learning_rate(.1) n_estimators(100) subsample(1) criterion(friedman_mse) min_samples_split(2) min_samples_leaf(1) 
min_weight_fraction_leaf(0) max_depth(3) min_impurity_decrease(0) init(None) random_state(rng) max_features(None) alpha(.9) 
max_leaf_nodes(None) warm_start(False) validation_fraction(.1) n_iter_no_change(None) tol(.0001) ccp_alpha(0) 


==> pystacked for Stata/Code/single_learner_2c.log.tex <==
. pystacked, type(reg) methods(lassocv) printopt
Default options: 
alphas(None) l1_ratio(1) eps(.001) n_alphas(100) fit_intercept(True) max_iter(1000) tol(.0001) 
n_jobs(None) positive(False) selection(cyclic) random_state(rng) 


==> pystacked for Stata/Code/single_learner_3.log.tex <==
. pystacked medh longi-medi if train,                        ///
>     type(regress) methods(gradboost)                       ///
>     cmdopt1(learning_rate(.01)) 
Single base learner: no stacking done.
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  gradboost      {\VBAR}      1.0000000
{\smallskip}
. predict double yhat_gb2 if !train
{\smallskip}
. pystacked medh longi-medi if train,                        ///
>     type(regress) methods(gradboost)                       ///
>     cmdopt1(learning_rate(.01) n_estimators(1000)) 
Single base learner: no stacking done.
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  gradboost      {\VBAR}      1.0000000
{\smallskip}
. predict double yhat_gb3 if !train
{\smallskip}


==> pystacked for Stata/Code/single_learner_3b.log.tex <==
. gen double res_gb1_sq=(medh-yhat_gb1){\caret}2 if !train
(15,448 missing values generated)
{\smallskip}
. gen double res_gb2_sq=(medh-yhat_gb2){\caret}2 if !train
(15,448 missing values generated)
{\smallskip}
. gen double res_gb3_sq=(medh-yhat_gb3){\caret}2 if !train
(15,448 missing values generated)
{\smallskip}
. sum res_gb* if !train
{\smallskip}
    Variable {\VBAR}        Obs        Mean    Std. dev.       Min        Max
\HLI{13}{\PLUS}\HLI{57}
  res_gb1_sq {\VBAR}      5,192    29.86727    83.17099   3.92e-06   1424.438
  res_gb2_sq {\VBAR}      5,192    71.10136    129.1446   4.56e-07   1230.348
  res_gb3_sq {\VBAR}      5,192    30.36929    82.88687   1.24e-06   1384.924
{\smallskip}


==> pystacked for Stata/Code/single_learner_4.log.tex <==
. pystacked medh longi-medi if train, type(reg) methods(lassocv)  
Single base learner: no stacking done.
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  lassocv        {\VBAR}      1.0000000
{\smallskip}
. predict double yhat_lasso1 if !train
{\smallskip}
. 
. pystacked medh longi-medi if train, type(reg) methods(lassocv) ///
>     pipe1(poly2)   
Single base learner: no stacking done.
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  lassocv        {\VBAR}      1.0000000
{\smallskip}
. predict double yhat_lasso2 if !train
{\smallskip}


==> pystacked for Stata/Code/single_learner_5.log.tex <==
. gen double res_lasso1_sq=(medh-yhat_lasso1){\caret}2 if !train
(15,448 missing values generated)
{\smallskip}
. gen double res_lasso2_sq=(medh-yhat_lasso2){\caret}2 if !train
(15,448 missing values generated)
{\smallskip}
. sum res_lasso1_sq res_lasso2_sq if !train
{\smallskip}
    Variable {\VBAR}        Obs        Mean    Std. dev.       Min        Max
\HLI{13}{\PLUS}\HLI{57}
res_lasso1{\tytilde}q {\VBAR}      5,192    47.00385    108.0759   8.43e-07   2392.572
res_lasso2{\tytilde}q {\VBAR}      5,192    43.81224    109.5096   6.75e-08    2563.15
{\smallskip}


==> pystacked for Stata/Code/stack_class_1.log.tex <==
. insheet using ///
>  https://archive.ics.uci.edu/ml/machine-learning-databases/spambase/spambase.data, ///
>  clear comma
(58 vars, 4,601 obs)
{\smallskip}
. set seed 42
{\smallskip}
. gen train=runiform()
{\smallskip}
. replace train=train<.75
(4,601 real changes made)


==> pystacked for Stata/Code/stack_class_2.log.tex <==
. pystacked v58 v1-v57                            || ///
>     m(logit) pipe(poly2)                        || ///
>     m(gradboost) opt(n_estimators(600))         || ///
>     m(gradboost) opt(n_estimators(1000))        || ///
>     m(nnet) opt(hidden_layer_sizes(5 5))        || ///
>     m(nnet) opt(hidden_layer_sizes(5))          || ///
>     if train, type(class) njobs(8) 
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  logit          {\VBAR}      0.0000000
  gradboost      {\VBAR}      0.4815155
  gradboost      {\VBAR}      0.3446655
  nnet           {\VBAR}      0.1131199
  nnet           {\VBAR}      0.0606992
{\smallskip}


==> pystacked for Stata/Code/stack_class_3.log.tex <==
. pystacked, table holdout
Number of holdout observations: 1133
{\smallskip}
Confusion matrix: In-Sample, CV, Holdout
\HLI{17}{\TOPT}\HLI{59}
  Method         {\VBAR} Weight      In-Sample             CV             Holdout
                 {\VBAR}             0       1         0       1         0       1
\HLI{17}{\PLUS}\HLI{59}
  STACKING     0 {\VBAR}    .      2079       6      2004      81       678      29
  STACKING     1 {\VBAR}    .         2    1381        77    1306        29     397
  logit        0 {\VBAR} 0.000     1265      88      1231      86       413      32
  logit        1 {\VBAR} 0.000      816    1299       850    1301       294     394
  gradboost    0 {\VBAR} 0.482     2078       9      2004      83       679      30
  gradboost    1 {\VBAR} 0.482        3    1378        77    1304        28     396
  gradboost    0 {\VBAR} 0.345     2079       1      2002      86       680      29
  gradboost    1 {\VBAR} 0.345        2    1386        79    1301        27     397
  nnet         0 {\VBAR} 0.113     1834      55      1975     132       617      28
  nnet         1 {\VBAR} 0.113      247    1332       106    1255        90     398
  nnet         0 {\VBAR} 0.061     2005     146      1924     116       671      51
  nnet         1 {\VBAR} 0.061       76    1241       157    1271        36     375
{\smallskip}


==> pystacked for Stata/Code/stack_class_4.log.tex <==
. pystacked,                                  ///
>     graph(subtitle(Spam data) scheme(sj))   ///
>     lgraph(plotopts(msymbol(i)              ///
>     ylabel(0 1, format(\%3.1f))) scheme(sj)) ///
>     holdout
Number of holdout observations: 1133
{\smallskip}


==> pystacked for Stata/Code/stack_reg_1.log.tex <==
. set seed 42
{\smallskip}
. pystacked medh longi-medi if train,                        ///
>     type(regress)                                          ///
>     methods(ols lassocv lassocv rf gradboost)              ///
>     pipe3(poly2) cmdopt5(learning_rate(0.01)               ///
>     n_estimators(1000))
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  ols            {\VBAR}      0.0000000
  lassocv        {\VBAR}      0.0000000
  lassocv        {\VBAR}      0.0000000
  rf             {\VBAR}      0.8382714
  gradboost      {\VBAR}      0.1617286
{\smallskip}


==> pystacked for Stata/Code/stack_reg_2.log.tex <==
. set seed 42
{\smallskip}
. pystacked medh longi-medi                                   || ///
>     m(ols)                                                  || ///
>     m(lassocv)                                              || ///
>     m(lassocv) pipe(poly2)                                  || ///
>     m(rf)                                                   || ///
>     m(gradboost) opt(learning_rate(0.01) n_estimators(1000))   ///
>     if train, type(regress) 
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  ols            {\VBAR}      0.0000000
  lassocv        {\VBAR}      0.0000000
  lassocv        {\VBAR}      0.0000000
  rf             {\VBAR}      0.8382714
  gradboost      {\VBAR}      0.1617286
{\smallskip}


==> pystacked for Stata/Code/stack_reg_3.log.tex <==
. predict double yhat, xb
{\smallskip}
. predict double ybase, basexb
{\smallskip}
. list yhat ybase* if _n <= 5
{\smallskip}
       {\TLC}\HLI{71}{\TRC}
       {\VBAR}      yhat      ybase1      ybase2      ybase3      ybase4      ybase5 {\VBAR}
       {\LFTT}\HLI{71}{\RGTT}
    1. {\VBAR} 42.875233   41.315834   41.193416    40.02005    43.16083   41.394926 {\VBAR}
    2. {\VBAR}  38.73664    41.45306   41.421461   44.443346   38.289107   41.056291 {\VBAR}
    3. {\VBAR}  40.68331   38.212036   38.154834   37.796287   41.268902   37.648071 {\VBAR}
    4. {\VBAR} 33.559085   32.332498   32.266321   32.546423     33.4869   33.933232 {\VBAR}
    5. {\VBAR} 24.190615   25.382839   25.369064   25.269325     23.8597   25.905815 {\VBAR}
       {\BLC}\HLI{71}{\BRC}


==> pystacked for Stata/Code/stack_reg_4.log.tex <==
. pystacked, graph(scheme(sj)) lgraph(scheme(sj)) holdout
Number of holdout observations: 5192
{\smallskip}


==> pystacked for Stata/Code/stack_reg_5.log.tex <==
. pystacked, table holdout
Number of holdout observations: 5192
{\smallskip}
RMSPE: In-Sample, CV, Holdout
\HLI{17}{\TOPT}\HLI{47}
  Method         {\VBAR} Weight   In-Sample        CV         Holdout
\HLI{17}{\PLUS}\HLI{47}
  STACKING       {\VBAR}    .        2.313        4.980        4.939
  ols            {\VBAR} 0.000       6.986        7.008        6.853
  lassocv        {\VBAR} 0.000       6.987        7.008        6.857
  lassocv        {\VBAR} 0.000       6.696        6.699        6.606
  rf             {\VBAR} 0.838       1.847        5.001        4.963
  gradboost      {\VBAR} 0.162       5.312        5.523        5.511
{\smallskip}


==> pystacked for Stata/Code/stack_reg_6.log.tex <==
. pystacked medh longi-medi                                   || ///
>     m(ols)                                                  || ///
>     m(ridgecv) xvars(c.(longi-medi)\#\#c.(longi-medi))        || ///
>     m(lassocv) xvars(c.(longi-medi)\#\#c.(longi-medi))        || ///
>     m(rf) opt(n_estimators(200))                            || ///
>     m(rf) opt(n_estimators(600))                            || ///
>     m(rf) opt(n_estimators(1000))                           || ///
>     m(gradboost) opt(n_estimators(200))                     || ///
>     m(gradboost) opt(n_estimators(600))                     || ///
>     m(gradboost) opt(n_estimators(1000))                    || ///
>     if train, type(regress) njobs(8)
{\smallskip}
Stacking weights:
\HLI{17}{\TOPT}\HLI{21}
  Method         {\VBAR}      Weight
\HLI{17}{\PLUS}\HLI{21}
  ols            {\VBAR}      0.0000000
  ridgecv        {\VBAR}      0.0000000
  lassocv        {\VBAR}      0.0000000
  rf             {\VBAR}      0.1343528
  rf             {\VBAR}      0.1923578
  rf             {\VBAR}      0.1299185
  gradboost      {\VBAR}      0.0000000
  gradboost      {\VBAR}      0.0000000
  gradboost      {\VBAR}      0.5433710
{\smallskip}

